FlowNet3D: Learning Scene Flow in 3D Point Clouds

Many applications in robotics and human-computer interaction can benefit from understanding 3D motion of points in a dynamic environment, widely noted as scene flow. While most previous methods focus on stereo and RGB-D images as input, few try to estimate scene flow directly from point clouds. In this work, we propose a novel deep neural network named $FlowNet3D$ that learns scene flow from point clouds in an end-to-end fashion. Our network simultaneously learns deep hierarchical features of point clouds and flow embeddings that represent point motions, supported by two newly proposed learning layers for point sets. We evaluate the network on both challenging synthetic data from FlyingThings3D and real Lidar scans from KITTI. Trained on synthetic data only, our network successfully generalizes to real scans, outperforming various baselines and showing competitive results to the prior art. We also demonstrate two applications of our scene flow output (scan registration and motion segmentation) to show its potential wide use cases.

==> design.tex <==


Before introducing our model, we firstly discuss design spaces of networks processing a pair of point clouds in estimating scene flow. The key aspects are \emph{where} and \emph{how} to mix the the two point clouds. Fig.~\ref{fig:mixture} illustrates three meta-architectures that mix signals at three different stages.


\paragraph{The Early Mixture model} combines raw input point clouds before any feature learning, with an encoder-decoder network M1 to predict per-point flow vector. Learning in this meta-architecture can be very challenging because raw point clouds provide little cue in how to associate them. 
How to represent the input is also not obvious as the two point clouds do not align/correspond.
A possible solution is to append a one-hot vector (with length two) as an extra feature to each point, with $(1,0)$ indicating the point is from the first set and $(0,1)$ for the other set. 

\paragraph{The Late Mixture model} firstly computes global features for each point cloud (with a shared sub-network M2) and then aggregates global features by concatenation. Per-point flow is estimated by combining local and global features with the network M3. As the two point clouds interact only at the level of global features, it is difficult to recover detailed local relations among the point clouds.

\paragraph{The Deep Mixture model} mixes two point clouds at intermediate feature levels. It firstly learns local point features on each input point clouds (with a shared sub-network M4), and then recover their relations from the both their local features and relative positions (M5) and propagate the information to the original points in the first set (M6). In this way, the interaction step (M5) benefits from both the spatial and feature cues in the two sets. However, the remaining challenge is how to design effective individual modules M4, M5 and M6, a topic we delve into in the next section.

\begin{comment}
In this section, we start by discussing design spaces of scene flow networks and showing three meta-architectures. Before diving into specific architectures, we review PointNet~\cite{qi2017pointnet}, a base learning module for point clouds. In the next section, we present FlowNet3D, an instantiation of one of the meta-architectures, with deep flow mixture and two novel neural network layers.

\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{mixture2.pdf}
\caption{\textbf{Three meta-architectures for scene flow network.} Inputs are two point clouds ($n$ points with $XYZ$ coordinates) from two frames, output is $n \times 3$ scene flow vector for each point in the first frame. Our FlowNet3D (Fig.~\ref{fig:network_architecture}) adopts the deep mixture scheme.}
\label{fig:mixture}
\end{figure*}


\paragraph{How to learn point cloud features?}
We follow the recently proposed PointNet++ architecture~\cite{qi2017pointnetplusplus}, a deep network that learns hierarchical point cloud features by recursively applying PointNets at local regions with increasing scales.
Another alternative is to use global features as learned from PointNet~\cite{qi2017pointnet} or EdgeConvNet~\cite{wang2018dynamic}, a choice that favors scenes with single objects but not ones with multiple objects moving independently.

\paragraph{Where to mix points from consecutive frames?} To estimate relative motion between points, we have to let them interact, or get mixed. We think there are at least three meta-architectures: \emph{early mixture}, \emph{late mixture} and \emph{deep mixture}, as shown in Fig.~\ref{fig:mixture}. An architecture with early mixture combines raw input point clouds before any feature learning. To note which frame a point comes from, one can add a one-hot vector (with length two) as an extra feature for each point. In contrast, late mixture only aggregates global features of the two point clouds. A processed global feature is further concatenated or propagated to each point to predict its flow. Instead of mixing points at raw level or global feature level, we can also mix them at intermediate levels, mixing locally learned features of point clouds, a process we call deep mixture.

\paragraph{How to mix them?} The simplest form of mixture is late mixture, global features from two point clouds are just concatenated and then further processed with fully connected layers. In both early mixture and deep mixture, we face two sets of point clouds (raw $XYZ$ in early and local point feature plus $XYZ$ for deep mixture). We will see in the next section that we can define a flow embedding layer that learns how to mix points for flow prediction. In experiments we will see that mixing points at the local feature level is much more effective than at the raw points level.


\subsection{Review of PointNet~\cite{qi2017pointnet}: A Base Learning Module for Point Clouds}
\label{sec:pointnet}
Recently, seminal work by Qi et al.~\cite{qi2017pointnet} proposed a novel neural network architecture for learning in point clouds. The architecture, named PointNet, in its simplest form, processes each point individually with a shared fully connected network across points, and then aggregate their outputs (point embeddings) through a max pooling function.
Due to the symmetry of pooling, the network is guaranteed to be invariant to the ordering of the points.

Mathematically, the base learning module is defined as following. Given a point cloud of $n$ orderless points: $\{x_1, x_2, ..., x_n\}$ with $x_i \in \mathbb{R}^d$,
our base learning module is a trainable set function $f: \mathcal{X} \rightarrow \mathbb{R}^c$

\begin{equation}
    f(x_1, x_2, ..., x_n) = \gamma \circ g(h(x_1), h(x_2), ..., h(x_n))
    \label{eq:pointnet}
\end{equation}
\noindent
where, as in~\cite{qi2017pointnet}, we use multi-layer perceptron for $h$, element-wise max pooling for $g$, and fully connected layers for $\gamma$ in further processing of the feature. 

In this work, we extensively use this \emph{pointnet}~\footnote{Lowercase to indicate it is not the original full network, but just a module.} module as a building block for our network, using it in many innovative ways specialized for scene flow estimation. See Fig.~\ref{fig:flow_embedding} Right (the gray block) and Fig.~\ref{fig:network_architecture} for detailed use cases.

\end{comment}

